Is there Anisotropy in Structural Bias?

Structural Bias (SB) is an important type of algorithmic deficiency within iterative optimisation heuristics. However, methods for detecting structural bias have not yet fully matured, and recent studies have uncovered many interesting questions. One of these is the question of how structural bias can be related to anisotropy. Intuitively, an algorithm that is not isotropic would be considered structurally biased. However, there have been cases where algorithms appear to only show SB in some dimensions. As such, we investigate whether these algorithms actually exhibit anisotropy, and how this impacts the detection of SB. We find that anisotropy is very rare, and even in cases where it is present, there are clear tests for SB which do not rely on any assumptions of isotropy, so we can safely expand the suite of SB tests to encompass these kinds of deficiencies not found by the original tests. We propose several additional testing procedures for SB detection and aim to motivate further research into the creation of a robust portfolio of tests. This is crucial since no single test will be able to work effectively with all types of SB we identify.

==> IMAGES/table_overview.tex <==
\begin{tabular}{lrrrrr}
\toprule
                       Name &  Rejections &  Rejections\_Transformed &  Rejections\_Spacing &  Fraction\_Corr\_Outliers &  Reject\_Aggregated \\
\midrule
          DE-best/2/bin (s) &          26 &                      26 &                   0 &                0.018391 &                  1 \\
          DE-best/2/bin (s) &          26 &                      26 &                   0 &                0.013793 &                  1 \\
          DE-best/1/exp (s) &          26 &                      26 &                   0 &                0.000000 &                  1 \\
      DE-curr-to-rand/1 (C) &          25 &                      30 &                   0 &                0.032184 &                  1 \\
                 Powell (C) &          25 &                       0 &                   0 &                0.018391 &                  1 \\
          DE-best/1/bin (s) &          24 &                      24 &                   0 &                0.011494 &                  1 \\
  DE-curr-to-best/1/bin (s) &          24 &                      24 &                   0 &                0.011494 &                  1 \\
  DE-curr-to-best/1/bin (s) &          24 &                      24 &                   0 &                0.011494 &                  1 \\
  DE-curr-to-best/1/bin (s) &          24 &                      24 &                   0 &                0.006897 &                  1 \\
         cDE-rand/2/bin (t) &          23 &                      30 &                   1 &                0.027586 &                  1 \\
  DE-curr-to-best/1/exp (s) &          22 &                      22 &                   0 &                0.013793 &                  1 \\
         cDE-rand/1/bin (s) &          22 &                      25 &                   0 &                0.006897 &                  1 \\
  DE-curr-to-best/1/exp (s) &          20 &                      20 &                   0 &                0.020690 &                  1 \\
             Rosenbrock (s) &          20 &                      20 &                   0 &                0.006897 &                  1 \\
 cDE-curr-to-best/1/bin (s) &          19 &                      20 &                   0 &                0.009195 &                  1 \\
  DE-curr-to-best/1/exp (s) &          17 &                      17 &                   0 &                0.013793 &                  1 \\
                 SPSAv2 (s) &          17 &                      17 &                   0 &                0.006897 &                  1 \\
                    RIS (m) &          13 &                       0 &                   0 &                0.032184 &                  1 \\
                   ISPO (s) &          11 &                      11 &                   1 &                0.016092 &                  1 \\
     cDE-curr-to-rand/1 (s) &          10 &                      12 &                   0 &                0.020690 &                  1 \\
                    RIS (C) &           9 &                       0 &                   0 &                0.016092 &                  1 \\
      DE-curr-to-rand/1 (m) &           9 &                      30 &                   0 &                0.013793 &                  1 \\
         cDE-rand/1/bin (t) &           7 &                      25 &                   0 &                0.013793 &                  1 \\
                   SPSA (C) &           0 &                       0 &                  30 &                0.105747 &                  0 \\
                   SPSA (m) &           0 &                       0 &                  30 &                0.087356 &                  0 \\
                   cPSO (C) &           0 &                       1 &                   0 &                0.052874 &                  1 \\
                    NMA (t) &           0 &                      30 &                   0 &                0.034483 &                  1 \\
                    NMA (m) &           0 &                      30 &                   0 &                0.034483 &                  1 \\
     cDE-curr-to-rand/1 (m) &           0 &                       0 &                   0 &                0.029885 &                  0 \\
                    cGA (i) &           0 &                       0 &                   0 &                0.027586 &                  1 \\
          DE-best/1/exp (m) &           0 &                       0 &                   0 &                0.027586 &                  0 \\
         cDE-best/2/exp (C) &           0 &                       0 &                   0 &                0.025287 &                  1 \\
               cDElight (d) &           0 &                       0 &                   0 &                0.025287 &                  1 \\
          DE-rand/2/bin (m) &           0 &                       0 &                   0 &                0.025287 &                  0 \\
          DE-rand/2/exp (m) &           0 &                       0 &                   0 &                0.025287 &                  0 \\
         cDE-rand/1/exp (t) &           0 &                       0 &                   0 &                0.022989 &                  1 \\
         cDE-rand/2/exp (m) &           0 &                       0 &                   0 &                0.022989 &                  0 \\
               cDElight (t) &           0 &                       0 &                   0 &                0.022989 &                  0 \\
          DE-best/1/bin (m) &           0 &                       0 &                   0 &                0.022989 &                  0 \\
          DE-best/1/exp (m) &           0 &                       0 &                   0 &                0.022989 &                  0 \\
  DE-rand-to-best/2/exp (d) &           0 &                       0 &                   0 &                0.022989 &                  0 \\
                    RIS (d) &           0 &                       0 &                   0 &                0.020690 &                  1 \\
         cDE-best/1/exp (m) &           0 &                       0 &                   0 &                0.020690 &                  0 \\
\bottomrule
\end{tabular}


==> MISC/DEMutationOperators.tex <==
\begin{itemize}
 \item {rand/1: \begin{equation}\label{eq:derand1}
           					    	\mathbf{x_m} = \mathbf{x_{r_1}}+F\left(\mathbf{x_{r_2}} - \mathbf{x_{r_3}}\right)
        		  \end{equation}}
    % \item { rand/2 \ak{not used here}: \begin{equation}\label{eq:derand2}
    %      					 	\mathbf{x_m} = \mathbf{x_{r_1}}+F\left(\mathbf{x_{r_2}} - \mathbf{x_{r_3}}\right) + F\left(\mathbf{x_{r_4}}-\mathbf{x_{r_5}}\right)
    %     			  \end{equation}}
    % \item {best/1 \ak{not used here}: \begin{equation}\label{eq:debest1}
    %         					\mathbf{x_m} = \mathbf{x_{best}}+F\left(\mathbf{x_{r_1}} - \mathbf{x_{r_2}}\right)
    %     		     \end{equation}}
    % \item {current-to-best/1 \ak{not used here}:\begin{equation}\label{eq:decurtobest}
    %         		                \mathbf{x_m} = \mathbf{x}+F \left(\mathbf{x_{best}} - \mathbf{x}\right)+F \left(\mathbf{x_{r_1}}-\mathbf{x_{r_2}}\right)
    %         		           \end{equation}}
\end{itemize}

==> MISC/newCommandsAndPackages.tex <==
\usepackage[dvips]{epsfig,graphicx}
\usepackage{times,subfigure,longtable,lscape,amssymb,amsbsy,times,fancyhdr,color,amsmath,latexsym,rotating,hhline,url,multirow} %eufrak
\usepackage{float,amsmath,graphicx,latexsym,amsfonts,amssymb,soul,wrapfig,dsfont}
\usepackage{caption,algorithm,algpseudocode}%algorithmic
\usepackage{textcomp}
\usepackage{hyperref}
\usepackage{amsmath}

\usepackage{float}
\usepackage{footnote}
\makesavenoteenv{tabular}
\makesavenoteenv{table}

\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


%\algdef{SE}[DOWHILE]{Do}{DoWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%
\newcommand{\ie}{i.e.,\,}
\newcommand{\ulc}[1]{\begin{picture}(#1,#1) \put(0,#1){\line(1,0){#1}} \put(0,0){\line(0,1){#1}} \end{picture}} 
\newcommand{\llc}[1]{\begin{picture}(#1,#1) \put(0,0){\line(1,0){#1}} \put(0,0){\line(0,1){#1}} \end{picture}} 
\newcommand{\urc}[1]{\begin{picture}(#1,#1) \put(0,#1){\line(1,0){#1}} \put(#1,0){\line(0,1){#1}} \end{picture}}
\newcommand{\lrc}[1]{\begin{picture}(#1,#1) \put(0,0){\line(1,0){#1}} \put(#1,0){\line(0,1){#1}} \end{picture}} 
\newcommand{\allc}[1]{\begin{picture}(#1,#1) \put(0,0){\line(1,0){#1}} \put(#1,0){\line(0,1){#1}} \put(0,#1){\line(1,0){#1}} \put(0,0){\line(0,1){#1}} \end{picture}} 


\newcommand{\version}{version of \today}

\setcounter{MaxMatrixCols}{10}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}

\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%

\usepackage{lipsum}


 \usepackage{tikz,pgfplots}
\pgfplotsset{compat=1.15}
\usepackage{gnuplottex}% use shutup


==> PSEUDOCODES/DE.tex <==
\begin{algorithm}[ht]
%\scriptsize
 \caption{Differential Evolution}\label{alg:DE}
\begin{center}
    % \captionof{algorithm}{Differential evolution}\label{alg:DE}
\begin{algorithmic}[0]
\State Initialise N$\in\mathbb{N}^+,F\in(0,2], Cr\in[0,1]$ \Comment{User defined}
\State $g\gets 1$\Comment{First generation}
\State $\text{POPULATION}_\text{g}\gets$ uniformly sample N individuals in \textbf{ D }$\subset\mathbb{R}^n$
\State $\mathbf{x_{best}}\gets$ fittest individual in $\text{POPULATION}_\text{g}$
\While{{condition on budget is not met}}
\State $\text{POPULATION}_{\text{g+1}}=\emptyset$
	\For{ each $\mathbf{x}\in\,\text{POPULATION}_\text{g}$}\Comment{i.e. N iterations}
		\State $\mathbf{x_m}\gets$ Mutation \Comment{e.g. equations \ref{eq:derand1} to \ref{eq:decurtobest}} 
		\State $\mathbf{x_{offspring}}\gets${CrossOver}$\left(\mathbf{x},\mathbf{x_m}\right)$\Comment{Algorithm \ref{alg:xobin} or \ref{alg:xoexp}}
		\If{$f\left(\mathbf{x_{offspring}}\right)\leq f\left(\mathbf{x}\right)$}%\Comment{Fill the next population} 
			\State $\text{POPULATION}_{\text{g+1}}=\text{POPULATION}_{\text{g+1}}\cup\{\mathbf{x_{offspring}}\}$
		\Else
			\State $\text{POPULATION}_{\text{g+1}}=\text{POPULATION}_{\text{g+1}}\cup\{\mathbf{x}\}$
		\EndIf
	\EndFor
	\State $g\gets g+1$\Comment{Replaces the old with the new population}
	\State $\mathbf{x_{best}}\gets$ fittest individual in $\text{POPULATION}_\text{g}$\Comment{Update best}
\EndWhile
\State \textbf{Output} {Best Individual} $\mathbf{x_{best}}$
\end{algorithmic}
\end{center}
\end{algorithm}

==> PSEUDOCODES/backupss.tex <==
 
% \begin{algorithm}
% \caption{Binomial crossover}\label{alg:xobin}
%  \begin{center}
%     %  \captionof{algorithm}{Binomial crossover}\label{alg:xobin}
% \begin{algorithmic}[0]
% \State \textbf{Input} two parents $\mathbf{x^1}$ and $\mathbf{x^2}$
% \State $\mathbf{x^{off}}\gets\mathbf{x^2}$
% \State $Index\gets \mathcal{I}\left(1,n\right)$\Comment{Random number in $\left[0,n\right]\subset\mathbb{N}$}%\footnote{Random integer uniformly distributed in $\left[0,n\right]\subset\mathbb{N}$}
% \State $\mathbf{x}_{(Index)}^{\mathbf{off}}\gets\mathbf{x}_{(Index)}^{\mathbf{1}}$
% \State $i\gets Index+1$
% \While{$\mathcal{U}$}\Comment{Random real number uniformly distributed in $\left[0,1\right]\subset\mathbb{R}$}%\footnote{Random number in $\left[0,1\right]\subset\mathbb{R}$}$\left(0,1\right)\leq CR\,\,||\,\,i\neq Index$}
% 		\State $\mathbf{x}_{(i)}^{\mathbf{off}}\gets\mathbf{{x}}_{(i)}^{\mathbf{1}}$
% 		\State $i\gets i+1$
% 		\If{$i>n$}
% 			\State $i\gets 1$
% 		\EndIf
% \EndWhile
% \State \textbf{Output} $\mathbf{x^{off}}$
% \end{algorithmic}
%  \end{center}
% \end{algorithm}


\begin{algorithm}
\caption{Binomial crossover}\label{alg:xobin}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} two parents $\mathbf{x_1}$ and $\mathbf{x_2}$\Comment{$\mathbf{x_1},\mathbf{x_2}\in$\textbf{ D }$\subset\mathbb{R}^n$}
\State $\mathbf{x_{offspring}}\gets\mathbf{x_1}$
% \State $\text{Index}\gets \mathcal{I}\left(1,n\right)$\Comment{$\mathcal{I}\left(1,n\right)$ is a random number in $\left[1,n\right]\subset\mathbb{N}$}%\footnote{Random integer uniformly
\State $\text{Index}\gets \mathcal{I}$\Comment{$\mathcal{I}$ is uniformly sampled in $\left[1,n\right]\subset\mathbb{N}$}%\footnote{Random integer uniformly
\For{$i=1,\dots,n$}
    % \If{$\mathcal{U}\left(0,1\right)<CR$ or $i==Index$} \Comment{$\mathcal{U}\left(1,n\right)$ is a random number in $\left[1,n\right]\subset\mathbb{R}$}
     \If{$\mathcal{U}\leq CR$ or $i=\text{Index}$} \Comment{$\mathcal{U}$ is uniformly sampled in $\left[0,1\right]\subset\mathbb{R}$}
% 		\State $\mathbf{x}_{\mathbf{offspring}}[i]\gets\mathbf{{x_2}}[i]$\Comment{exchange the $i^{th}$ component}
		\State $\mathbf{x}^{(i)}_{\mathbf{offspring}}\gets\mathbf{x}^{(i)}_\mathbf{2}$\Comment{exchange the $i^{th}$ component}
	\EndIf
\EndFor
\State \textbf{Output} $\mathbf{x_{offspring}}$
\end{algorithmic}
 \end{center}
\end{algorithm}


% \begin{algorithm}
% \caption{Discard correction}
% \begin{center}
%     %\captionof{algorithm}{Discard correction}\label{alg:discard}
% \begin{algorithmic}[1]
% \State \textbf{Input} a solution $\mathbf{x}$ and problem's boundaries \Comment{$\mathbf{x}\in\mathbb{R}^n$ but domain is $\textbf{ D }\subset\mathbb{R}^n$}
% \State $i\gets 0$
% \While{$\text{out}==\text{false}$}
% 	\State \textit{l}$\gets${i-th lower bound}
% 	\State \textit{u}$\gets${i-th upper bound}
% 	\If{$x_{(i)} > u \text{ or } x_{(i)} < l $}
% 		\State Break \Comment{do not evaluate its fitness}
% 	\Else
% 	\State $i\gets i+1$
% 	\EndIf
% \EndWhile
% \State \textbf{Output} $\mathbf{x}$
% |state \hl{I believe it is pointless to give this details for this correction, thus I produced the shorter pseudocode below... what do you think? perhaps the is not even need of pseudocode for this one}
% \end{algorithmic}
% \end{center}
% \end{algorithm}

\begin{algorithm}
\caption{Discard correction}\label{alg:discard}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} a solution $\mathbf{x}$ and problem's boundaries \Comment{$\mathbf{x}\in\mathbb{R}^n$ but domain is $\textbf{ D }\subset\mathbb{R}^n$}
\If{$\mathbf{x}\not\in\mathbf{D}$}
    \State $\mathbf{x}\gets$ a selected parent%\hl{radonmly chosen parent? resampled?}
\EndIf
\State \textbf{Output} $\mathbf{x}$ \Comment{No fitness functional call required}
\end{algorithmic}
\end{center}
\end{algorithm}

% \begin{algorithm}
%   \caption{Exponential crossover}\label{alg:xoexp}
% \begin{center}
%     % \captionof{algorithm}{Exponential crossover}\label{alg:xoexp}
% \begin{algorithmic}[0]
% \State \textbf{Input} two parents $\mathbf{x^1}$ and $\mathbf{x^2}$
% \State $\mathbf{x^{off}}\gets\mathbf{x^2}$
% \State $Index\gets \mathcal{I}\left(1,n\right)$\footnote{Random number in $\left[0,n\right]\subset\mathbb{N}$}\Comment{Random integer number uniformly distributed in $\left[0,n\right]\subset\mathbb{N}$}
% \State $\mathbf{x}_{(Index)}^{\mathbf{off}}\gets\mathbf{x}_{(Index)}^{\mathbf{1}}$
% \State $i\gets Index+1$
% \While{$\mathcal{U}$}\Comment{Random number uniformly distributed in $\left[0,1\right]\subset\mathbb{R}$}%\footnote{Random number in $\left[0,1\right]\subset\mathbb{R}$}$\left(0,1\right)\leq CR\,\,||\,\,i\neq Index$}
% 		\State $\mathbf{x}_{(i)}^{\mathbf{off}}\gets\mathbf{x}_{(i)}^{\mathbf{1}}$
% 		\State $i\gets i+1$
% 		\If{$i>n$}
% 			\State $i\gets 1$
% 		\EndIf
% \EndWhile
% \State \textbf{Output} $\mathbf{x^{off}}$
% \end{algorithmic}
% \end{center}
% \end{algorithm}

\begin{algorithm}
   \caption{Exponential crossover}\label{alg:xoexp}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} two parents $\mathbf{x_1}$ and $\mathbf{x_2}$\Comment{$\mathbf{x_1},\mathbf{x_2}\in$\textbf{ D }$\subset\mathbb{R}^n$}
\State $\mathbf{x_{offspring}}\gets\mathbf{x_1}$
\State $i,\text{Index}\gets \mathcal{I}$\Comment{$\mathcal{I}$ is uniformly sampled in $\left[1,n\right]\subset\mathbb{N}$}
% \State $\mathbf{x}_{(Index)}^{\mathbf{off}}\gets\mathbf{x}_{(Index)}^{\mathbf{1}}$
% \State $i\gets Index+1$
\Do
\State $\mathbf{x}^{(i)}_\mathbf{offspring}\gets\mathbf{x}^{(i)}_\mathbf{2}$\Comment{exchange the $i^{th}$ component}
\State $i\gets i+1$
\If{$i>n$}
			\State $i\gets 1$
		\EndIf
\doWhile{$\mathcal{U}\leq CR$ and $i\neq \text{Index}$} \Comment{$\mathcal{U}$ is uniformly distributed in $\left[0,1\right]\subset\mathbb{R}$}
\State \textbf{Output} $\mathbf{x_{offspring}}$
\end{algorithmic}
\end{center}
\end{algorithm}

% \begin{algorithm}
%   \caption{Exponential crossover}\label{alg:xoexp}
% \begin{center}
%     % \captionof{algorithm}{Exponential crossover}\label{alg:xoexp}
% \begin{algorithmic}[0]
% \State \textbf{Input} two parents $\mathbf{x^1}$ and $\mathbf{x^2}$
% \State $\mathbf{x^{off}}\gets\mathbf{x^2}$
% \State $Index\gets \mathcal{I}\left(1,n\right)$\footnote{Random number in $\left[0,n\right]\subset\mathbb{N}$}\Comment{Random integer number uniformly distributed in $\left[0,n\right]\subset\mathbb{N}$}
% \State $\mathbf{x}_{(Index)}^{\mathbf{off}}\gets\mathbf{x}_{(Index)}^{\mathbf{1}}$
% \State $i\gets Index+1$
% \While{$\mathcal{U}$}\Comment{Random number uniformly distributed in $\left[0,1\right]\subset\mathbb{R}$}%\footnote{Random number in $\left[0,1\right]\subset\mathbb{R}$}$\left(0,1\right)\leq CR\,\,||\,\,i\neq Index$}
% 		\State $\mathbf{x}_{(i)}^{\mathbf{off}}\gets\mathbf{x}_{(i)}^{\mathbf{1}}$
% 		\State $i\gets i+1$
% 		\If{$i>n$}
% 			\State $i\gets 1$
% 		\EndIf
% \EndWhile
% \State \textbf{Output} $\mathbf{x^{off}}$
% \end{algorithmic}
% \end{center}
% \end{algorithm}

\begin{algorithm}
   \caption{Exponential crossover}\label{alg:xoexp}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} two parents $\mathbf{x_1}$ and $\mathbf{x_2}$\Comment{$\mathbf{x_1},\mathbf{x_2}\in$\textbf{ D }$\subset\mathbb{R}^n$}
\State $\mathbf{x_{offspring}}\gets\mathbf{x_1}$
\State $i,\text{Index}\gets \mathcal{I}$\Comment{$\mathcal{I}$ is uniformly sampled in $\left[1,n\right]\subset\mathbb{N}$}
% \State $\mathbf{x}_{(Index)}^{\mathbf{off}}\gets\mathbf{x}_{(Index)}^{\mathbf{1}}$
% \State $i\gets Index+1$
\Do
\State $\mathbf{x}^{(i)}_\mathbf{offspring}\gets\mathbf{x}^{(i)}_\mathbf{2}$\Comment{exchange the $i^{th}$ component}
\State $i\gets i+1$
\If{$i>n$}
			\State $i\gets 1$
		\EndIf
\doWhile{$\mathcal{U}\leq CR$ and $i\neq \text{Index}$} \Comment{$\mathcal{U}$ is uniformly distributed in $\left[0,1\right]\subset\mathbb{R}$}
\State \textbf{Output} $\mathbf{x_{offspring}}$
\end{algorithmic}
\end{center}
\end{algorithm}

% \begin{algorithm}
% \caption{Saturation correction}\label{alg:saturation}
% \begin{center}
% \begin{algorithmic}%[0]
%     %\Function{Saturate}{$\mathbf{x}$}
% \State \textbf{Input} a point $\mathbf{x}\in\textbf{ D }$\subset\mathbb{R}^n$}$
% \For{$i=1:n$}
% 	\State {l}$\gets${i-th lower bound}
% 	\State {u}$\gets${i-th upper bound}
% 	\If{$\mathbf{x}_i >$\textit{u}}
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets$u
% 	\ElsIf{$\mathbf{x_{norm}}<$\textit{l}}
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets$l
% 	\Else
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets \mathbf{x}^{(i)}$
% 	\EndIf		
% \EndFor
% \State \textbf{Output} $\mathbf{x_{saturated}}$
% %\EndFunction
% \end{algorithmic}
% \end{center}
% \end{algorithm}
\begin{algorithm}
\caption{Saturation correction}\label{alg:saturation}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} a solution $\mathbf{x}$ and problem's boundaries \Comment{$\mathbf{x}\in\mathbb{R}^n$ but domain is $\textbf{ D }\subset\mathbb{R}^n$}
\For{$i=1,\dots,n$}
	\State {l}$\gets${$i^{th}$ lower bound}
	\State {u}$\gets${$i^{th}$ upper bound}
	\If{$\mathbf{x}_i >$\textit{u}}
		\State $\mathbf{x}^{(i)}_\mathbf{saturated}\gets$ u\Comment{saturate the $i^{th}$ component to the upper-bound}
	\ElsIf{$\mathbf{x_{norm}}<$\textit{l}}
		\State $\mathbf{x}^{(i)}_\mathbf{saturated}\gets$ l \Comment{saturate the $i^{th}$ component to the lower-bound}
	\Else
		\State $\mathbf{x}^{(i)}_\mathbf{saturated}\gets\mathbf{x}^{(i)}$\Comment{keep the original $i^{th}$ component}
	\EndIf		
\EndFor
\State \textbf{Output} $\mathbf{x_{saturated}}$
%\EndFunction
\end{algorithmic}
\end{center}
\end{algorithm}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% FABIO  14/07/2017  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \noindent\begin{minipage}{.5\textwidth}
% \captionof{algorithm}{Saturation correction}\label{alg:saturation}
% \begin{algorithmic}[0]
% %\Function{Saturate}{$\mathbf{x}$}
% \State \textbf{Input} a point $\mathbf{x}\in\mathbb{R}^n$
% \For{$i=1:n$}
% 	\State {l}$\gets${i-th lower bound}
% 	\State {u}$\gets${i-th upper bound}
% 	\If{$\mathbf{x}_i >$\textit{u}}
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets$u
% 	\ElsIf{$\mathbf{x_{norm}}<$\textit{l}}
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets$l
% 	\Else
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets \mathbf{x}^{(i)}$
% 	\EndIf		
% \EndFor
% \State \textbf{Output} $\mathbf{x_{saturated}}$
% %\EndFunction
% \end{algorithmic}
% \end{minipage}%
% \begin{minipage}{.7\textwidth}
% \captionof{algorithm}{Toroidal correction}\label{alg:toro}
% \begin{algorithmic}[0]
% %\Function{ToroidalCorrection}{$\mathbf{x}$}
% \State \textbf{Input} a point $\mathbf{x}\in\mathbb{R}^n$
% \For{$i=1:n$}
% 	\State {l}$\gets${i-th lower bound}
% 	\State {u}$\gets${i-th upper bound}
% 	\State $\delta\gets${u - l}
% 	\State $\mathbf{x_{norm}}^{(i)} \gets \frac{\mathbf{x}^{(i)}-\textit{l}}{\delta}$
% 	\State $x_{r}\gets${rounds} $\mathbf{x}^{(i)}$ {to the nearest integer towards $0$}
% 	\If{$\mathbf{x_{norm}}^{(i)} > 1$}%\Comment{Toroidal transformation}
% 		\State $\mathbf{x_{norm}}^{(i)}\gets \mathbf{x_{norm}}^{(i)}-x_r$
% 	\ElsIf{$\mathbf{x_{norm}} < 0$}
% 		\State $\mathbf{x_{norm}}^{(i)}\gets 1 - \left|\mathbf{x_{norm}}^{(i)}-x_r\right|$
% 	\EndIf	
% 	\State $\mathbf{x_{corrected}}^{(i)}\gets{l}+\mathbf{x_{norm}}^{(i)}\cdot\delta$
% \EndFor
% \State \textbf{Output} $\mathbf{x_{corrected}}$
% %\EndFunction
% \end{algorithmic}
% \end{minipage}

%
%%
%
% \begin{minipage}{.5\textwidth}
% \captionof{algorithm}{Penalty correction}\label{alg:penalty}
% \begin{algorithmic}[0]
% \State \textbf{Input} {a point} $\mathbf{x}\in\mathbb{R}^n$
% \State $\text{out}\gets\text{false}$
% \State $i\gets 0$
% \While{$\text{out}==\text{false}$}
% 	\State \textit{l}$\gets${i-th lower bound}
% 	\State \textit{u}$\gets${i-th upper bound}
% 	\If{$x_{(i)} > u \text{ or } x_{(i)} < l $}
% 		\State $\text{out}\gets\text{true}$
% 		\State $\mathbf{x}\text{ will get a fitness value } > 1$
% 	\Else
% 	\State $i\gets i+1$
% 	\EndIf
% \EndWhile
% \State \textbf{Output} $\mathbf{x}$
% \end{algorithmic}
% \end{minipage}
% %
% \begin{minipage}{.5\textwidth}
% \captionof{algorithm}{Discard correction}\label{alg:discard}
% \begin{algorithmic}[0]
% \State \textbf{Input} {a point} $\mathbf{x}\in\mathbb{R}^n$
% \State $i\gets 0$
% \While{$\text{out}==\text{false}$}
% 	\State \textit{l}$\gets${i-th lower bound}
% 	\State \textit{u}$\gets${i-th upper bound}
% 	\If{$x_{(i)} > u \text{ or } x_{(i)} < l $}
% 		\State Break \small{(do not evaluate its fitness)}
% 	\Else
% 	\State $i\gets i+1$
% 	\EndIf
% \EndWhile
% \State \textbf{Output} $\mathbf{x}$
% \end{algorithmic}
% \end{minipage}
% %% 


% \captionof{algorithm}{Penalty correction}\label{alg:penalty}

% \begin{algorithm}
% \caption{Toroidal correction}\label{alg:toro}
% \begin{center}
% %\captionof{algorithm}{Toroidal correction}\label{alg:toro}
% \begin{algorithmic}[1]
% %\Function{ToroidalCorrection}{$\mathbf{x}$}
% \State \textbf{Input} a solution $\mathbf{x}$ \Comment{$\mathbf{x}\in\textbf{ D }\subset\mathbb{R}^n$}
% \For{$i=1,\dots,n$}
% 	\State {l}$\gets${$i^{th}$ lower bound}
% 	\State {u}$\gets${$i^{th}$$ upper bound}
% 	\State $\delta\gets${u - l}
% 	\State $\mathbf{x_{norm}}^{(i)} \gets \frac{\mathbf{x}^{(i)}-\textit{l}}{\delta}$
% 	\State $x_{r}\gets${rounds} $\mathbf{x}^{(i)}$ {to the nearest integer towards $0$}
% 	\If{$\mathbf{x_{norm}}^{(i)} > 1$}%\Comment{Toroidal transformation}
% 		\State $\mathbf{x_{norm}}^{(i)}\gets \mathbf{x_{norm}}^{(i)}-x_r$
% 	\ElsIf{$\mathbf{x_{norm}} < 0$}
% 		\State $\mathbf{x_{norm}}^{(i)}\gets 1 - \left|\mathbf{x_{norm}}^{(i)}-x_r\right|$
% 	\EndIf	
% 	\State $\mathbf{x_{corrected}}^{(i)}\gets{l}+\mathbf{x_{norm}}^{(i)}\cdot\delta$
% \EndFor
% \State \textbf{Output} $\mathbf{x_{corrected}}$
% %\EndFunction
% \end{algorithmic}
% \end{center}
% \end{algorithm}

\begin{algorithm}
\caption{Toroidal correction}\label{alg:toro}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} a solution $\mathbf{x}$ and problem's boundaries \Comment{$\mathbf{x}\in\mathbb{R}^n$ but domain is $\textbf{ D }\subset\mathbb{R}^n$}
\For{$i=1,\dots,n$}
	\State {l}$\gets${$i^{th}$ lower bound}
	\State {u}$\gets${$i^{th}$ upper bound}
	\State $x_N\gets\frac{\mathbf{x}^{(i)}-\textit{l}}{u-l}$\Comment{normalise $i^{th}$ component of $\mathbf{x}$ in $[0,1]$}
	\State $x_{R}\gets${rounds} $\mathbf{x}^{(i)}$ {to the nearest integer towards $0$}
	\If{$x_N > 1$}%\Comment{Toroidal transformation}
		\State $x_N\gets x_N-x_R$
	\ElsIf{$x_N < 0$}
		\State $x_N\gets 1 - \left|x_N-x_R\right|$
	\EndIf	
	\State $\mathbf{x_{corrected}}^{(i)}\gets{l}+X_N\cdot\left(u-l\right)$\Comment{scale the corrected value back to \textbf{D}}
\EndFor
\State \textbf{Output} $\mathbf{x_{corrected}}$
%\EndFunction
\end{algorithmic}
\end{center}
\end{algorithm}

==> PSEUDOCODES/bin.tex <==
\begin{algorithm}[ht]
\caption{Binomial crossover}\label{alg:xobin}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} two parents $\mathbf{x_1}$ and $\mathbf{x_2}$\Comment{$\mathbf{x_1},\mathbf{x_2}\in$\textbf{ D }$\subset\mathbb{R}^n$}
 \State A random index $\mathcal{I}$ is uniformly drawn in $\left[1,n\right]\subset\mathbb{N}$
\For{$i=1,2,3,\dots,n$} 
\State A random value $\mathcal{U}$ is uniformly drawn in $\left[0,1\right]\subset\mathbb{R}$
     \If{$\mathcal{U}\leq Cr$ or $i==\mathcal{I}$}\Comment{$Cr\in[0,1]$ is user defined}
		\State $\mathbf{x}_\mathbf{1}[i]\gets\mathbf{x}_\mathbf{2}[i]$\Comment{Exchange the $i^{th}$ component}
	\EndIf
\EndFor
 \State \textbf{Output} $\mathbf{x}_\mathbf{1}$
\end{algorithmic}
\end{center}
\end{algorithm}

==> PSEUDOCODES/discard.tex <==

\begin{algorithm}[H]
\caption{Discard correction}\label{alg:discard}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} a solution $\mathbf{x}$ and problem's boundaries \Comment{$\mathbf{x}\in\mathbb{R}^n$ but domain is $\textbf{ D }\subset\mathbb{R}^n$}
\If{$\mathbf{x}\not\in\mathbf{D}$}
    \State $\mathbf{x}\gets$ a selected parent%\hl{radonmly chosen parent? resampled?}
\EndIf
\State \textbf{Output} $\mathbf{x}$ \Comment{No fitness functional call required}
\end{algorithmic}
\end{center}
\end{algorithm}



==> PSEUDOCODES/exp.tex <==
\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%
\begin{algorithm}[ht!]
  \caption{Exponential crossover}\label{alg:xoexp}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} two parents $\mathbf{x_1}$ and $\mathbf{x_2}$\Comment{$\mathbf{x_1},\mathbf{x_2}\in$\textbf{ D }$\subset\mathbb{R}^n$}
\State A random index $\mathcal{I}$ is uniformly drawn in $\left[1,n\right]\subset\mathbb{N}$
\State $i\gets\mathcal{I}$
\Do
\State $\mathbf{x}_\mathbf{1}[i]\gets\mathbf{x}_\mathbf{2}[i]$\Comment{exchange the $i^{th}$ component}
\State $i\gets i+1$
\If{$i>n$}
			\State $i\gets 1$
		\EndIf
\State A random value $\mathcal{U}$ is uniformly drawn in $\left[0,1\right]\subset\mathbb{R}$
\doWhile{$\mathcal{U}\leq CR$ and $i\neq \text{Index}$}\Comment{$Cr\in[0,1]$ is user defined} 
\State \textbf{Output} $\mathbf{x_{1}}$
\end{algorithmic}
\end{center}
\end{algorithm}

==> PSEUDOCODES/penalty.tex <==

\begin{algorithm}[H]\caption{Penalty correction}\label{alg:penalty}
\begin{center}
    \begin{algorithmic}[0]
\State \textbf{Input} {a point} $\mathbf{x}\in\mathbb{R}^n$
\State $\text{out}\gets\text{false}$
\State $i\gets 0$
\While{$\text{out}==\text{false}$}
	\State \textit{l}$\gets${i-th lower bound}
	\State \textit{u}$\gets${i-th upper bound}
	\If{$x_{(i)} > u \text{ or } x_{(i)} < l $}
		\State $\text{out}\gets\text{true}$
		\State $\mathbf{x}\text{ will get a fitness value } > 1$
	\Else
	\State $i\gets i+1$
	\EndIf
\EndWhile
\State \textbf{Output} $\mathbf{x}$
\end{algorithmic}

\end{center}
\end{algorithm}

==> PSEUDOCODES/saturation.tex <==

\begin{algorithm}[H]
\caption{Saturation correction}\label{alg:saturation}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} a solution $\mathbf{x}$ and problem's boundaries \Comment{$\mathbf{x}\in\mathbb{R}^n$ but domain is $\textbf{ D }\subset\mathbb{R}^n$}
\For{$i=1,\dots,n$}
	\State {l}$\gets${$i^{th}$ lower bound}
	\State {u}$\gets${$i^{th}$ upper bound}
	\If{$\mathbf{x}_i >$\textit{u}}
		\State $\mathbf{x}^{(i)}_\mathbf{saturated}\gets$ u\Comment{saturate the $i^{th}$ component to the upper-bound}
	\ElsIf{$\mathbf{x_{saturated}}<$\textit{l}}
		\State $\mathbf{x}^{(i)}_\mathbf{saturated}\gets$ l \Comment{saturate the $i^{th}$ component to the lower-bound}
	\Else
		\State $\mathbf{x}^{(i)}_\mathbf{saturated}\gets\mathbf{x}^{(i)}$\Comment{keep the original $i^{th}$ component}
	\EndIf		
\EndFor
\State \textbf{Output} $\mathbf{x_{saturated}}$
%\EndFunction
\end{algorithmic}
\end{center}
\end{algorithm}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% FABIO  14/07/2017  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \noindent\begin{minipage}{.5\textwidth}
% \captionof{algorithm}{Saturation correction}\label{alg:saturation}
% \begin{algorithmic}[0]
% %\Function{Saturate}{$\mathbf{x}$}
% \State \textbf{Input} a point $\mathbf{x}\in\mathbb{R}^n$
% \For{$i=1:n$}
% 	\State {l}$\gets${i-th lower bound}
% 	\State {u}$\gets${i-th upper bound}
% 	\If{$\mathbf{x}_i >$\textit{u}}
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets$u
% 	\ElsIf{$\mathbf{x_{norm}}<$\textit{l}}
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets$l
% 	\Else
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets \mathbf{x}^{(i)}$
% 	\EndIf		
% \EndFor
% \State \textbf{Output} $\mathbf{x_{saturated}}$
% %\EndFunction
% \end{algorithmic}
% \end{minipage}%
% \begin{minipage}{.7\textwidth}
% \captionof{algorithm}{Toroidal correction}\label{alg:toro}
% \begin{algorithmic}[0]
% %\Function{ToroidalCorrection}{$\mathbf{x}$}
% \State \textbf{Input} a point $\mathbf{x}\in\mathbb{R}^n$
% \For{$i=1:n$}
% 	\State {l}$\gets${i-th lower bound}
% 	\State {u}$\gets${i-th upper bound}
% 	\State $\delta\gets${u - l}
% 	\State $\mathbf{x_{norm}}^{(i)} \gets \frac{\mathbf{x}^{(i)}-\textit{l}}{\delta}$
% 	\State $x_{r}\gets${rounds} $\mathbf{x}^{(i)}$ {to the nearest integer towards $0$}
% 	\If{$\mathbf{x_{norm}}^{(i)} > 1$}%\Comment{Toroidal transformation}
% 		\State $\mathbf{x_{norm}}^{(i)}\gets \mathbf{x_{norm}}^{(i)}-x_r$
% 	\ElsIf{$\mathbf{x_{norm}} < 0$}
% 		\State $\mathbf{x_{norm}}^{(i)}\gets 1 - \left|\mathbf{x_{norm}}^{(i)}-x_r\right|$
% 	\EndIf	
% 	\State $\mathbf{x_{corrected}}^{(i)}\gets{l}+\mathbf{x_{norm}}^{(i)}\cdot\delta$
% \EndFor
% \State \textbf{Output} $\mathbf{x_{corrected}}$
% %\EndFunction
% \end{algorithmic}
% \end{minipage}

%
%%
%
% \begin{minipage}{.5\textwidth}
% \captionof{algorithm}{Penalty correction}\label{alg:penalty}
% \begin{algorithmic}[0]
% \State \textbf{Input} {a point} $\mathbf{x}\in\mathbb{R}^n$
% \State $\text{out}\gets\text{false}$
% \State $i\gets 0$
% \While{$\text{out}==\text{false}$}
% 	\State \textit{l}$\gets${i-th lower bound}
% 	\State \textit{u}$\gets${i-th upper bound}
% 	\If{$x_{(i)} > u \text{ or } x_{(i)} < l $}
% 		\State $\text{out}\gets\text{true}$
% 		\State $\mathbf{x}\text{ will get a fitness value } > 1$
% 	\Else
% 	\State $i\gets i+1$
% 	\EndIf
% \EndWhile
% \State \textbf{Output} $\mathbf{x}$
% \end{algorithmic}
% \end{minipage}
% %
% \begin{minipage}{.5\textwidth}
% \captionof{algorithm}{Discard correction}\label{alg:discard}
% \begin{algorithmic}[0]
% \State \textbf{Input} {a point} $\mathbf{x}\in\mathbb{R}^n$
% \State $i\gets 0$
% \While{$\text{out}==\text{false}$}
% 	\State \textit{l}$\gets${i-th lower bound}
% 	\State \textit{u}$\gets${i-th upper bound}
% 	\If{$x_{(i)} > u \text{ or } x_{(i)} < l $}
% 		\State Break \small{(do not evaluate its fitness)}
% 	\Else
% 	\State $i\gets i+1$
% 	\EndIf
% \EndWhile
% \State \textbf{Output} $\mathbf{x}$
% \end{algorithmic}
% \end{minipage}
% %% 


% \captionof{algorithm}{Penalty correction}\label{alg:penalty}

==> PSEUDOCODES/toroidal.tex <==

\begin{algorithm}[H]
\caption{Toroidal correction}\label{alg:toro}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} a solution $\mathbf{x}$ and problem's boundaries \Comment{$\mathbf{x}\in\mathbb{R}^n$ but domain is $\textbf{ D }\subset\mathbb{R}^n$}
\For{$i=1,\dots,n$}
	\State {l}$\gets${$i^{th}$ lower bound}
	\State {u}$\gets${$i^{th}$ upper bound}
	\State $x_N\gets\frac{\mathbf{x}^{(i)}-\textit{l}}{u-l}$\Comment{normalise $i^{th}$ component of $\mathbf{x}$ in $[0,1]$}
	\State $x_{R}\gets${rounds} $\mathbf{x}^{(i)}$ {to the nearest integer towards $0$}
	\If{$x_N > 1$}%\Comment{Toroidal transformation}
		\State $x_N\gets x_N-x_R$
	\ElsIf{$x_N < 0$}
		\State $x_N\gets 1 - \left|x_N-x_R\right|$
	\EndIf	
	\State $\mathbf{x_{corrected}}^{(i)}\gets{l}+X_N\cdot\left(u-l\right)$\Comment{scale the corrected value back to \textbf{D}}
\EndFor
\State \textbf{Output} $\mathbf{x_{corrected}}$
%\EndFunction
\end{algorithmic}
\end{center}
\end{algorithm}

==> old/MISC/DEMutationOperators.tex <==
\begin{itemize}
 \item {rand/1: \begin{equation}\label{eq:derand1}
           					    	\mathbf{x_m} = \mathbf{x_{r_1}}+F\left(\mathbf{x_{r_2}} - \mathbf{x_{r_3}}\right)
        		  \end{equation}}
    % \item { rand/2 \ak{not used here}: \begin{equation}\label{eq:derand2}
    %      					 	\mathbf{x_m} = \mathbf{x_{r_1}}+F\left(\mathbf{x_{r_2}} - \mathbf{x_{r_3}}\right) + F\left(\mathbf{x_{r_4}}-\mathbf{x_{r_5}}\right)
    %     			  \end{equation}}
    % \item {best/1 \ak{not used here}: \begin{equation}\label{eq:debest1}
    %         					\mathbf{x_m} = \mathbf{x_{best}}+F\left(\mathbf{x_{r_1}} - \mathbf{x_{r_2}}\right)
    %     		     \end{equation}}
    % \item {current-to-best/1 \ak{not used here}:\begin{equation}\label{eq:decurtobest}
    %         		                \mathbf{x_m} = \mathbf{x}+F \left(\mathbf{x_{best}} - \mathbf{x}\right)+F \left(\mathbf{x_{r_1}}-\mathbf{x_{r_2}}\right)
    %         		           \end{equation}}
\end{itemize}

==> old/MISC/newCommandsAndPackages.tex <==
\usepackage[dvips]{epsfig,graphicx}
\usepackage{times,subfigure,longtable,lscape,amssymb,amsbsy,times,fancyhdr,color,amsmath,latexsym,rotating,hhline,url,multirow} %eufrak
\usepackage{float,amsmath,graphicx,latexsym,amsfonts,amssymb,soul,wrapfig,dsfont}
\usepackage{caption,algorithm,algpseudocode}%algorithmic
\usepackage{textcomp}
\usepackage{hyperref}
\usepackage{amsmath}

\usepackage{float}
\usepackage{footnote}
\makesavenoteenv{tabular}
\makesavenoteenv{table}

\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%


%\algdef{SE}[DOWHILE]{Do}{DoWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%
\newcommand{\ie}{i.e.,\,}
\newcommand{\ulc}[1]{\begin{picture}(#1,#1) \put(0,#1){\line(1,0){#1}} \put(0,0){\line(0,1){#1}} \end{picture}} 
\newcommand{\llc}[1]{\begin{picture}(#1,#1) \put(0,0){\line(1,0){#1}} \put(0,0){\line(0,1){#1}} \end{picture}} 
\newcommand{\urc}[1]{\begin{picture}(#1,#1) \put(0,#1){\line(1,0){#1}} \put(#1,0){\line(0,1){#1}} \end{picture}}
\newcommand{\lrc}[1]{\begin{picture}(#1,#1) \put(0,0){\line(1,0){#1}} \put(#1,0){\line(0,1){#1}} \end{picture}} 
\newcommand{\allc}[1]{\begin{picture}(#1,#1) \put(0,0){\line(1,0){#1}} \put(#1,0){\line(0,1){#1}} \put(0,#1){\line(1,0){#1}} \put(0,0){\line(0,1){#1}} \end{picture}} 


\newcommand{\version}{version of \today}

\setcounter{MaxMatrixCols}{10}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}

\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%

\usepackage{lipsum}


 \usepackage{tikz,pgfplots}
\pgfplotsset{compat=1.15}
\usepackage{gnuplottex}% use shutup


==> old/PSEUDOCODES/DE.tex <==
\begin{algorithm}[ht]
%\scriptsize
 \caption{Differential Evolution}\label{alg:DE}
\begin{center}
    % \captionof{algorithm}{Differential evolution}\label{alg:DE}
\begin{algorithmic}[0]
\State Initialise N$\in\mathbb{N}^+,F\in(0,2], Cr\in[0,1]$ \Comment{User defined}
\State $g\gets 1$\Comment{First generation}
\State $\text{POPULATION}_\text{g}\gets$ uniformly sample N individuals in \textbf{ D }$\subset\mathbb{R}^n$
\State $\mathbf{x_{best}}\gets$ fittest individual in $\text{POPULATION}_\text{g}$
\While{{condition on budget is not met}}
\State $\text{POPULATION}_{\text{g+1}}=\emptyset$
	\For{ each $\mathbf{x}\in\,\text{POPULATION}_\text{g}$}\Comment{i.e. N iterations}
		\State $\mathbf{x_m}\gets$ Mutation \Comment{e.g. equations \ref{eq:derand1} to \ref{eq:decurtobest}} 
		\State $\mathbf{x_{offspring}}\gets${CrossOver}$\left(\mathbf{x},\mathbf{x_m}\right)$\Comment{Algorithm \ref{alg:xobin} or \ref{alg:xoexp}}
		\If{$f\left(\mathbf{x_{offspring}}\right)\leq f\left(\mathbf{x}\right)$}%\Comment{Fill the next population} 
			\State $\text{POPULATION}_{\text{g+1}}=\text{POPULATION}_{\text{g+1}}\cup\{\mathbf{x_{offspring}}\}$
		\Else
			\State $\text{POPULATION}_{\text{g+1}}=\text{POPULATION}_{\text{g+1}}\cup\{\mathbf{x}\}$
		\EndIf
	\EndFor
	\State $g\gets g+1$\Comment{Replaces the old with the new population}
	\State $\mathbf{x_{best}}\gets$ fittest individual in $\text{POPULATION}_\text{g}$\Comment{Update best}
\EndWhile
\State \textbf{Output} {Best Individual} $\mathbf{x_{best}}$
\end{algorithmic}
\end{center}
\end{algorithm}

==> old/PSEUDOCODES/backupss.tex <==

% \begin{algorithm}
% \caption{Binomial crossover}\label{alg:xobin}
%  \begin{center}
%     %  \captionof{algorithm}{Binomial crossover}\label{alg:xobin}
% \begin{algorithmic}[0]
% \State \textbf{Input} two parents $\mathbf{x^1}$ and $\mathbf{x^2}$
% \State $\mathbf{x^{off}}\gets\mathbf{x^2}$
% \State $Index\gets \mathcal{I}\left(1,n\right)$\Comment{Random number in $\left[0,n\right]\subset\mathbb{N}$}%\footnote{Random integer uniformly distributed in $\left[0,n\right]\subset\mathbb{N}$}
% \State $\mathbf{x}_{(Index)}^{\mathbf{off}}\gets\mathbf{x}_{(Index)}^{\mathbf{1}}$
% \State $i\gets Index+1$
% \While{$\mathcal{U}$}\Comment{Random real number uniformly distributed in $\left[0,1\right]\subset\mathbb{R}$}%\footnote{Random number in $\left[0,1\right]\subset\mathbb{R}$}$\left(0,1\right)\leq CR\,\,||\,\,i\neq Index$}
% 		\State $\mathbf{x}_{(i)}^{\mathbf{off}}\gets\mathbf{{x}}_{(i)}^{\mathbf{1}}$
% 		\State $i\gets i+1$
% 		\If{$i>n$}
% 			\State $i\gets 1$
% 		\EndIf
% \EndWhile
% \State \textbf{Output} $\mathbf{x^{off}}$
% \end{algorithmic}
%  \end{center}
% \end{algorithm}


\begin{algorithm}
\caption{Binomial crossover}\label{alg:xobin}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} two parents $\mathbf{x_1}$ and $\mathbf{x_2}$\Comment{$\mathbf{x_1},\mathbf{x_2}\in$\textbf{ D }$\subset\mathbb{R}^n$}
\State $\mathbf{x_{offspring}}\gets\mathbf{x_1}$
% \State $\text{Index}\gets \mathcal{I}\left(1,n\right)$\Comment{$\mathcal{I}\left(1,n\right)$ is a random number in $\left[1,n\right]\subset\mathbb{N}$}%\footnote{Random integer uniformly
\State $\text{Index}\gets \mathcal{I}$\Comment{$\mathcal{I}$ is uniformly sampled in $\left[1,n\right]\subset\mathbb{N}$}%\footnote{Random integer uniformly
\For{$i=1,\dots,n$}
    % \If{$\mathcal{U}\left(0,1\right)<CR$ or $i==Index$} \Comment{$\mathcal{U}\left(1,n\right)$ is a random number in $\left[1,n\right]\subset\mathbb{R}$}
     \If{$\mathcal{U}\leq CR$ or $i=\text{Index}$} \Comment{$\mathcal{U}$ is uniformly sampled in $\left[0,1\right]\subset\mathbb{R}$}
% 		\State $\mathbf{x}_{\mathbf{offspring}}[i]\gets\mathbf{{x_2}}[i]$\Comment{exchange the $i^{th}$ component}
		\State $\mathbf{x}^{(i)}_{\mathbf{offspring}}\gets\mathbf{x}^{(i)}_\mathbf{2}$\Comment{exchange the $i^{th}$ component}
	\EndIf
\EndFor
\State \textbf{Output} $\mathbf{x_{offspring}}$
\end{algorithmic}
 \end{center}
\end{algorithm}


% \begin{algorithm}
% \caption{Discard correction}
% \begin{center}
%     %\captionof{algorithm}{Discard correction}\label{alg:discard}
% \begin{algorithmic}[1]
% \State \textbf{Input} a solution $\mathbf{x}$ and problem's boundaries \Comment{$\mathbf{x}\in\mathbb{R}^n$ but domain is $\textbf{ D }\subset\mathbb{R}^n$}
% \State $i\gets 0$
% \While{$\text{out}==\text{false}$}
% 	\State \textit{l}$\gets${i-th lower bound}
% 	\State \textit{u}$\gets${i-th upper bound}
% 	\If{$x_{(i)} > u \text{ or } x_{(i)} < l $}
% 		\State Break \Comment{do not evaluate its fitness}
% 	\Else
% 	\State $i\gets i+1$
% 	\EndIf
% \EndWhile
% \State \textbf{Output} $\mathbf{x}$
% |state \hl{I believe it is pointless to give this details for this correction, thus I produced the shorter pseudocode below... what do you think? perhaps the is not even need of pseudocode for this one}
% \end{algorithmic}
% \end{center}
% \end{algorithm}

\begin{algorithm}
\caption{Discard correction}\label{alg:discard}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} a solution $\mathbf{x}$ and problem's boundaries \Comment{$\mathbf{x}\in\mathbb{R}^n$ but domain is $\textbf{ D }\subset\mathbb{R}^n$}
\If{$\mathbf{x}\not\in\mathbf{D}$}
    \State $\mathbf{x}\gets$ a selected parent%\hl{radonmly chosen parent? resampled?}
\EndIf
\State \textbf{Output} $\mathbf{x}$ \Comment{No fitness functional call required}
\end{algorithmic}
\end{center}
\end{algorithm}

% \begin{algorithm}
%   \caption{Exponential crossover}\label{alg:xoexp}
% \begin{center}
%     % \captionof{algorithm}{Exponential crossover}\label{alg:xoexp}
% \begin{algorithmic}[0]
% \State \textbf{Input} two parents $\mathbf{x^1}$ and $\mathbf{x^2}$
% \State $\mathbf{x^{off}}\gets\mathbf{x^2}$
% \State $Index\gets \mathcal{I}\left(1,n\right)$\footnote{Random number in $\left[0,n\right]\subset\mathbb{N}$}\Comment{Random integer number uniformly distributed in $\left[0,n\right]\subset\mathbb{N}$}
% \State $\mathbf{x}_{(Index)}^{\mathbf{off}}\gets\mathbf{x}_{(Index)}^{\mathbf{1}}$
% \State $i\gets Index+1$
% \While{$\mathcal{U}$}\Comment{Random number uniformly distributed in $\left[0,1\right]\subset\mathbb{R}$}%\footnote{Random number in $\left[0,1\right]\subset\mathbb{R}$}$\left(0,1\right)\leq CR\,\,||\,\,i\neq Index$}
% 		\State $\mathbf{x}_{(i)}^{\mathbf{off}}\gets\mathbf{x}_{(i)}^{\mathbf{1}}$
% 		\State $i\gets i+1$
% 		\If{$i>n$}
% 			\State $i\gets 1$
% 		\EndIf
% \EndWhile
% \State \textbf{Output} $\mathbf{x^{off}}$
% \end{algorithmic}
% \end{center}
% \end{algorithm}

\begin{algorithm}
   \caption{Exponential crossover}\label{alg:xoexp}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} two parents $\mathbf{x_1}$ and $\mathbf{x_2}$\Comment{$\mathbf{x_1},\mathbf{x_2}\in$\textbf{ D }$\subset\mathbb{R}^n$}
\State $\mathbf{x_{offspring}}\gets\mathbf{x_1}$
\State $i,\text{Index}\gets \mathcal{I}$\Comment{$\mathcal{I}$ is uniformly sampled in $\left[1,n\right]\subset\mathbb{N}$}
% \State $\mathbf{x}_{(Index)}^{\mathbf{off}}\gets\mathbf{x}_{(Index)}^{\mathbf{1}}$
% \State $i\gets Index+1$
\Do
\State $\mathbf{x}^{(i)}_\mathbf{offspring}\gets\mathbf{x}^{(i)}_\mathbf{2}$\Comment{exchange the $i^{th}$ component}
\State $i\gets i+1$
\If{$i>n$}
			\State $i\gets 1$
		\EndIf
\doWhile{$\mathcal{U}\leq CR$ and $i\neq \text{Index}$} \Comment{$\mathcal{U}$ is uniformly distributed in $\left[0,1\right]\subset\mathbb{R}$}
\State \textbf{Output} $\mathbf{x_{offspring}}$
\end{algorithmic}
\end{center}
\end{algorithm}

% \begin{algorithm}
%   \caption{Exponential crossover}\label{alg:xoexp}
% \begin{center}
%     % \captionof{algorithm}{Exponential crossover}\label{alg:xoexp}
% \begin{algorithmic}[0]
% \State \textbf{Input} two parents $\mathbf{x^1}$ and $\mathbf{x^2}$
% \State $\mathbf{x^{off}}\gets\mathbf{x^2}$
% \State $Index\gets \mathcal{I}\left(1,n\right)$\footnote{Random number in $\left[0,n\right]\subset\mathbb{N}$}\Comment{Random integer number uniformly distributed in $\left[0,n\right]\subset\mathbb{N}$}
% \State $\mathbf{x}_{(Index)}^{\mathbf{off}}\gets\mathbf{x}_{(Index)}^{\mathbf{1}}$
% \State $i\gets Index+1$
% \While{$\mathcal{U}$}\Comment{Random number uniformly distributed in $\left[0,1\right]\subset\mathbb{R}$}%\footnote{Random number in $\left[0,1\right]\subset\mathbb{R}$}$\left(0,1\right)\leq CR\,\,||\,\,i\neq Index$}
% 		\State $\mathbf{x}_{(i)}^{\mathbf{off}}\gets\mathbf{x}_{(i)}^{\mathbf{1}}$
% 		\State $i\gets i+1$
% 		\If{$i>n$}
% 			\State $i\gets 1$
% 		\EndIf
% \EndWhile
% \State \textbf{Output} $\mathbf{x^{off}}$
% \end{algorithmic}
% \end{center}
% \end{algorithm}

\begin{algorithm}
   \caption{Exponential crossover}\label{alg:xoexp}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} two parents $\mathbf{x_1}$ and $\mathbf{x_2}$\Comment{$\mathbf{x_1},\mathbf{x_2}\in$\textbf{ D }$\subset\mathbb{R}^n$}
\State $\mathbf{x_{offspring}}\gets\mathbf{x_1}$
\State $i,\text{Index}\gets \mathcal{I}$\Comment{$\mathcal{I}$ is uniformly sampled in $\left[1,n\right]\subset\mathbb{N}$}
% \State $\mathbf{x}_{(Index)}^{\mathbf{off}}\gets\mathbf{x}_{(Index)}^{\mathbf{1}}$
% \State $i\gets Index+1$
\Do
\State $\mathbf{x}^{(i)}_\mathbf{offspring}\gets\mathbf{x}^{(i)}_\mathbf{2}$\Comment{exchange the $i^{th}$ component}
\State $i\gets i+1$
\If{$i>n$}
			\State $i\gets 1$
		\EndIf
\doWhile{$\mathcal{U}\leq CR$ and $i\neq \text{Index}$} \Comment{$\mathcal{U}$ is uniformly distributed in $\left[0,1\right]\subset\mathbb{R}$}
\State \textbf{Output} $\mathbf{x_{offspring}}$
\end{algorithmic}
\end{center}
\end{algorithm}

% \begin{algorithm}
% \caption{Saturation correction}\label{alg:saturation}
% \begin{center}
% \begin{algorithmic}%[0]
%     %\Function{Saturate}{$\mathbf{x}$}
% \State \textbf{Input} a point $\mathbf{x}\in\textbf{ D }$\subset\mathbb{R}^n$}$
% \For{$i=1:n$}
% 	\State {l}$\gets${i-th lower bound}
% 	\State {u}$\gets${i-th upper bound}
% 	\If{$\mathbf{x}_i >$\textit{u}}
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets$u
% 	\ElsIf{$\mathbf{x_{norm}}<$\textit{l}}
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets$l
% 	\Else
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets \mathbf{x}^{(i)}$
% 	\EndIf		
% \EndFor
% \State \textbf{Output} $\mathbf{x_{saturated}}$
% %\EndFunction
% \end{algorithmic}
% \end{center}
% \end{algorithm}
\begin{algorithm}
\caption{Saturation correction}\label{alg:saturation}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} a solution $\mathbf{x}$ and problem's boundaries \Comment{$\mathbf{x}\in\mathbb{R}^n$ but domain is $\textbf{ D }\subset\mathbb{R}^n$}
\For{$i=1,\dots,n$}
	\State {l}$\gets${$i^{th}$ lower bound}
	\State {u}$\gets${$i^{th}$ upper bound}
	\If{$\mathbf{x}_i >$\textit{u}}
		\State $\mathbf{x}^{(i)}_\mathbf{saturated}\gets$ u\Comment{saturate the $i^{th}$ component to the upper-bound}
	\ElsIf{$\mathbf{x_{norm}}<$\textit{l}}
		\State $\mathbf{x}^{(i)}_\mathbf{saturated}\gets$ l \Comment{saturate the $i^{th}$ component to the lower-bound}
	\Else
		\State $\mathbf{x}^{(i)}_\mathbf{saturated}\gets\mathbf{x}^{(i)}$\Comment{keep the original $i^{th}$ component}
	\EndIf		
\EndFor
\State \textbf{Output} $\mathbf{x_{saturated}}$
%\EndFunction
\end{algorithmic}
\end{center}
\end{algorithm}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% FABIO  14/07/2017  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \noindent\begin{minipage}{.5\textwidth}
% \captionof{algorithm}{Saturation correction}\label{alg:saturation}
% \begin{algorithmic}[0]
% %\Function{Saturate}{$\mathbf{x}$}
% \State \textbf{Input} a point $\mathbf{x}\in\mathbb{R}^n$
% \For{$i=1:n$}
% 	\State {l}$\gets${i-th lower bound}
% 	\State {u}$\gets${i-th upper bound}
% 	\If{$\mathbf{x}_i >$\textit{u}}
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets$u
% 	\ElsIf{$\mathbf{x_{norm}}<$\textit{l}}
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets$l
% 	\Else
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets \mathbf{x}^{(i)}$
% 	\EndIf		
% \EndFor
% \State \textbf{Output} $\mathbf{x_{saturated}}$
% %\EndFunction
% \end{algorithmic}
% \end{minipage}%
% \begin{minipage}{.7\textwidth}
% \captionof{algorithm}{Toroidal correction}\label{alg:toro}
% \begin{algorithmic}[0]
% %\Function{ToroidalCorrection}{$\mathbf{x}$}
% \State \textbf{Input} a point $\mathbf{x}\in\mathbb{R}^n$
% \For{$i=1:n$}
% 	\State {l}$\gets${i-th lower bound}
% 	\State {u}$\gets${i-th upper bound}
% 	\State $\delta\gets${u - l}
% 	\State $\mathbf{x_{norm}}^{(i)} \gets \frac{\mathbf{x}^{(i)}-\textit{l}}{\delta}$
% 	\State $x_{r}\gets${rounds} $\mathbf{x}^{(i)}$ {to the nearest integer towards $0$}
% 	\If{$\mathbf{x_{norm}}^{(i)} > 1$}%\Comment{Toroidal transformation}
% 		\State $\mathbf{x_{norm}}^{(i)}\gets \mathbf{x_{norm}}^{(i)}-x_r$
% 	\ElsIf{$\mathbf{x_{norm}} < 0$}
% 		\State $\mathbf{x_{norm}}^{(i)}\gets 1 - \left|\mathbf{x_{norm}}^{(i)}-x_r\right|$
% 	\EndIf	
% 	\State $\mathbf{x_{corrected}}^{(i)}\gets{l}+\mathbf{x_{norm}}^{(i)}\cdot\delta$
% \EndFor
% \State \textbf{Output} $\mathbf{x_{corrected}}$
% %\EndFunction
% \end{algorithmic}
% \end{minipage}

%
%%
%
% \begin{minipage}{.5\textwidth}
% \captionof{algorithm}{Penalty correction}\label{alg:penalty}
% \begin{algorithmic}[0]
% \State \textbf{Input} {a point} $\mathbf{x}\in\mathbb{R}^n$
% \State $\text{out}\gets\text{false}$
% \State $i\gets 0$
% \While{$\text{out}==\text{false}$}
% 	\State \textit{l}$\gets${i-th lower bound}
% 	\State \textit{u}$\gets${i-th upper bound}
% 	\If{$x_{(i)} > u \text{ or } x_{(i)} < l $}
% 		\State $\text{out}\gets\text{true}$
% 		\State $\mathbf{x}\text{ will get a fitness value } > 1$
% 	\Else
% 	\State $i\gets i+1$
% 	\EndIf
% \EndWhile
% \State \textbf{Output} $\mathbf{x}$
% \end{algorithmic}
% \end{minipage}
% %
% \begin{minipage}{.5\textwidth}
% \captionof{algorithm}{Discard correction}\label{alg:discard}
% \begin{algorithmic}[0]
% \State \textbf{Input} {a point} $\mathbf{x}\in\mathbb{R}^n$
% \State $i\gets 0$
% \While{$\text{out}==\text{false}$}
% 	\State \textit{l}$\gets${i-th lower bound}
% 	\State \textit{u}$\gets${i-th upper bound}
% 	\If{$x_{(i)} > u \text{ or } x_{(i)} < l $}
% 		\State Break \small{(do not evaluate its fitness)}
% 	\Else
% 	\State $i\gets i+1$
% 	\EndIf
% \EndWhile
% \State \textbf{Output} $\mathbf{x}$
% \end{algorithmic}
% \end{minipage}
% %% 


% \captionof{algorithm}{Penalty correction}\label{alg:penalty}

% \begin{algorithm}
% \caption{Toroidal correction}\label{alg:toro}
% \begin{center}
% %\captionof{algorithm}{Toroidal correction}\label{alg:toro}
% \begin{algorithmic}[1]
% %\Function{ToroidalCorrection}{$\mathbf{x}$}
% \State \textbf{Input} a solution $\mathbf{x}$ \Comment{$\mathbf{x}\in\textbf{ D }\subset\mathbb{R}^n$}
% \For{$i=1,\dots,n$}
% 	\State {l}$\gets${$i^{th}$ lower bound}
% 	\State {u}$\gets${$i^{th}$$ upper bound}
% 	\State $\delta\gets${u - l}
% 	\State $\mathbf{x_{norm}}^{(i)} \gets \frac{\mathbf{x}^{(i)}-\textit{l}}{\delta}$
% 	\State $x_{r}\gets${rounds} $\mathbf{x}^{(i)}$ {to the nearest integer towards $0$}
% 	\If{$\mathbf{x_{norm}}^{(i)} > 1$}%\Comment{Toroidal transformation}
% 		\State $\mathbf{x_{norm}}^{(i)}\gets \mathbf{x_{norm}}^{(i)}-x_r$
% 	\ElsIf{$\mathbf{x_{norm}} < 0$}
% 		\State $\mathbf{x_{norm}}^{(i)}\gets 1 - \left|\mathbf{x_{norm}}^{(i)}-x_r\right|$
% 	\EndIf	
% 	\State $\mathbf{x_{corrected}}^{(i)}\gets{l}+\mathbf{x_{norm}}^{(i)}\cdot\delta$
% \EndFor
% \State \textbf{Output} $\mathbf{x_{corrected}}$
% %\EndFunction
% \end{algorithmic}
% \end{center}
% \end{algorithm}

\begin{algorithm}
\caption{Toroidal correction}\label{alg:toro}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} a solution $\mathbf{x}$ and problem's boundaries \Comment{$\mathbf{x}\in\mathbb{R}^n$ but domain is $\textbf{ D }\subset\mathbb{R}^n$}
\For{$i=1,\dots,n$}
	\State {l}$\gets${$i^{th}$ lower bound}
	\State {u}$\gets${$i^{th}$ upper bound}
	\State $x_N\gets\frac{\mathbf{x}^{(i)}-\textit{l}}{u-l}$\Comment{normalise $i^{th}$ component of $\mathbf{x}$ in $[0,1]$}
	\State $x_{R}\gets${rounds} $\mathbf{x}^{(i)}$ {to the nearest integer towards $0$}
	\If{$x_N > 1$}%\Comment{Toroidal transformation}
		\State $x_N\gets x_N-x_R$
	\ElsIf{$x_N < 0$}
		\State $x_N\gets 1 - \left|x_N-x_R\right|$
	\EndIf	
	\State $\mathbf{x_{corrected}}^{(i)}\gets{l}+X_N\cdot\left(u-l\right)$\Comment{scale the corrected value back to \textbf{D}}
\EndFor
\State \textbf{Output} $\mathbf{x_{corrected}}$
%\EndFunction
\end{algorithmic}
\end{center}
\end{algorithm}

==> old/PSEUDOCODES/bin.tex <==
\begin{algorithm}[ht]
\caption{Binomial crossover}\label{alg:xobin}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} two parents $\mathbf{x_1}$ and $\mathbf{x_2}$\Comment{$\mathbf{x_1},\mathbf{x_2}\in$\textbf{ D }$\subset\mathbb{R}^n$}
 \State A random index $\mathcal{I}$ is uniformly drawn in $\left[1,n\right]\subset\mathbb{N}$
\For{$i=1,2,3,\dots,n$} 
\State A random value $\mathcal{U}$ is uniformly drawn in $\left[0,1\right]\subset\mathbb{R}$
     \If{$\mathcal{U}\leq Cr$ or $i==\mathcal{I}$}\Comment{$Cr\in[0,1]$ is user defined}
		\State $\mathbf{x}_\mathbf{1}[i]\gets\mathbf{x}_\mathbf{2}[i]$\Comment{Exchange the $i^{th}$ component}
	\EndIf
\EndFor
 \State \textbf{Output} $\mathbf{x}_\mathbf{1}$
\end{algorithmic}
\end{center}
\end{algorithm}

==> old/PSEUDOCODES/discard.tex <==

\begin{algorithm}[H]
\caption{Discard correction}\label{alg:discard}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} a solution $\mathbf{x}$ and problem's boundaries \Comment{$\mathbf{x}\in\mathbb{R}^n$ but domain is $\textbf{ D }\subset\mathbb{R}^n$}
\If{$\mathbf{x}\not\in\mathbf{D}$}
    \State $\mathbf{x}\gets$ a selected parent%\hl{radonmly chosen parent? resampled?}
\EndIf
\State \textbf{Output} $\mathbf{x}$ \Comment{No fitness functional call required}
\end{algorithmic}
\end{center}
\end{algorithm}



==> old/PSEUDOCODES/exp.tex <==
\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%
\begin{algorithm}[ht!]
  \caption{Exponential crossover}\label{alg:xoexp}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} two parents $\mathbf{x_1}$ and $\mathbf{x_2}$\Comment{$\mathbf{x_1},\mathbf{x_2}\in$\textbf{ D }$\subset\mathbb{R}^n$}
\State A random index $\mathcal{I}$ is uniformly drawn in $\left[1,n\right]\subset\mathbb{N}$
\State $i\gets\mathcal{I}$
\Do
\State $\mathbf{x}_\mathbf{1}[i]\gets\mathbf{x}_\mathbf{2}[i]$\Comment{exchange the $i^{th}$ component}
\State $i\gets i+1$
\If{$i>n$}
			\State $i\gets 1$
		\EndIf
\State A random value $\mathcal{U}$ is uniformly drawn in $\left[0,1\right]\subset\mathbb{R}$
\doWhile{$\mathcal{U}\leq CR$ and $i\neq \text{Index}$}\Comment{$Cr\in[0,1]$ is user defined} 
\State \textbf{Output} $\mathbf{x_{1}}$
\end{algorithmic}
\end{center}
\end{algorithm}

==> old/PSEUDOCODES/penalty.tex <==

\begin{algorithm}[H]\caption{Penalty correction}\label{alg:penalty}
\begin{center}
    \begin{algorithmic}[0]
\State \textbf{Input} {a point} $\mathbf{x}\in\mathbb{R}^n$
\State $\text{out}\gets\text{false}$
\State $i\gets 0$
\While{$\text{out}==\text{false}$}
	\State \textit{l}$\gets${i-th lower bound}
	\State \textit{u}$\gets${i-th upper bound}
	\If{$x_{(i)} > u \text{ or } x_{(i)} < l $}
		\State $\text{out}\gets\text{true}$
		\State $\mathbf{x}\text{ will get a fitness value } > 1$
	\Else
	\State $i\gets i+1$
	\EndIf
\EndWhile
\State \textbf{Output} $\mathbf{x}$
\end{algorithmic}

\end{center}
\end{algorithm}

==> old/PSEUDOCODES/saturation.tex <==

\begin{algorithm}[H]
\caption{Saturation correction}\label{alg:saturation}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} a solution $\mathbf{x}$ and problem's boundaries \Comment{$\mathbf{x}\in\mathbb{R}^n$ but domain is $\textbf{ D }\subset\mathbb{R}^n$}
\For{$i=1,\dots,n$}
	\State {l}$\gets${$i^{th}$ lower bound}
	\State {u}$\gets${$i^{th}$ upper bound}
	\If{$\mathbf{x}_i >$\textit{u}}
		\State $\mathbf{x}^{(i)}_\mathbf{saturated}\gets$ u\Comment{saturate the $i^{th}$ component to the upper-bound}
	\ElsIf{$\mathbf{x_{saturated}}<$\textit{l}}
		\State $\mathbf{x}^{(i)}_\mathbf{saturated}\gets$ l \Comment{saturate the $i^{th}$ component to the lower-bound}
	\Else
		\State $\mathbf{x}^{(i)}_\mathbf{saturated}\gets\mathbf{x}^{(i)}$\Comment{keep the original $i^{th}$ component}
	\EndIf		
\EndFor
\State \textbf{Output} $\mathbf{x_{saturated}}$
%\EndFunction
\end{algorithmic}
\end{center}
\end{algorithm}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% FABIO  14/07/2017  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \noindent\begin{minipage}{.5\textwidth}
% \captionof{algorithm}{Saturation correction}\label{alg:saturation}
% \begin{algorithmic}[0]
% %\Function{Saturate}{$\mathbf{x}$}
% \State \textbf{Input} a point $\mathbf{x}\in\mathbb{R}^n$
% \For{$i=1:n$}
% 	\State {l}$\gets${i-th lower bound}
% 	\State {u}$\gets${i-th upper bound}
% 	\If{$\mathbf{x}_i >$\textit{u}}
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets$u
% 	\ElsIf{$\mathbf{x_{norm}}<$\textit{l}}
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets$l
% 	\Else
% 		\State $\mathbf{x_{saturated}}^{(i)}\gets \mathbf{x}^{(i)}$
% 	\EndIf		
% \EndFor
% \State \textbf{Output} $\mathbf{x_{saturated}}$
% %\EndFunction
% \end{algorithmic}
% \end{minipage}%
% \begin{minipage}{.7\textwidth}
% \captionof{algorithm}{Toroidal correction}\label{alg:toro}
% \begin{algorithmic}[0]
% %\Function{ToroidalCorrection}{$\mathbf{x}$}
% \State \textbf{Input} a point $\mathbf{x}\in\mathbb{R}^n$
% \For{$i=1:n$}
% 	\State {l}$\gets${i-th lower bound}
% 	\State {u}$\gets${i-th upper bound}
% 	\State $\delta\gets${u - l}
% 	\State $\mathbf{x_{norm}}^{(i)} \gets \frac{\mathbf{x}^{(i)}-\textit{l}}{\delta}$
% 	\State $x_{r}\gets${rounds} $\mathbf{x}^{(i)}$ {to the nearest integer towards $0$}
% 	\If{$\mathbf{x_{norm}}^{(i)} > 1$}%\Comment{Toroidal transformation}
% 		\State $\mathbf{x_{norm}}^{(i)}\gets \mathbf{x_{norm}}^{(i)}-x_r$
% 	\ElsIf{$\mathbf{x_{norm}} < 0$}
% 		\State $\mathbf{x_{norm}}^{(i)}\gets 1 - \left|\mathbf{x_{norm}}^{(i)}-x_r\right|$
% 	\EndIf	
% 	\State $\mathbf{x_{corrected}}^{(i)}\gets{l}+\mathbf{x_{norm}}^{(i)}\cdot\delta$
% \EndFor
% \State \textbf{Output} $\mathbf{x_{corrected}}$
% %\EndFunction
% \end{algorithmic}
% \end{minipage}

%
%%
%
% \begin{minipage}{.5\textwidth}
% \captionof{algorithm}{Penalty correction}\label{alg:penalty}
% \begin{algorithmic}[0]
% \State \textbf{Input} {a point} $\mathbf{x}\in\mathbb{R}^n$
% \State $\text{out}\gets\text{false}$
% \State $i\gets 0$
% \While{$\text{out}==\text{false}$}
% 	\State \textit{l}$\gets${i-th lower bound}
% 	\State \textit{u}$\gets${i-th upper bound}
% 	\If{$x_{(i)} > u \text{ or } x_{(i)} < l $}
% 		\State $\text{out}\gets\text{true}$
% 		\State $\mathbf{x}\text{ will get a fitness value } > 1$
% 	\Else
% 	\State $i\gets i+1$
% 	\EndIf
% \EndWhile
% \State \textbf{Output} $\mathbf{x}$
% \end{algorithmic}
% \end{minipage}
% %
% \begin{minipage}{.5\textwidth}
% \captionof{algorithm}{Discard correction}\label{alg:discard}
% \begin{algorithmic}[0]
% \State \textbf{Input} {a point} $\mathbf{x}\in\mathbb{R}^n$
% \State $i\gets 0$
% \While{$\text{out}==\text{false}$}
% 	\State \textit{l}$\gets${i-th lower bound}
% 	\State \textit{u}$\gets${i-th upper bound}
% 	\If{$x_{(i)} > u \text{ or } x_{(i)} < l $}
% 		\State Break \small{(do not evaluate its fitness)}
% 	\Else
% 	\State $i\gets i+1$
% 	\EndIf
% \EndWhile
% \State \textbf{Output} $\mathbf{x}$
% \end{algorithmic}
% \end{minipage}
% %% 


% \captionof{algorithm}{Penalty correction}\label{alg:penalty}

==> old/PSEUDOCODES/toroidal.tex <==

\begin{algorithm}[H]
\caption{Toroidal correction}\label{alg:toro}
\begin{center}
\begin{algorithmic}[0]
\State \textbf{Input} a solution $\mathbf{x}$ and problem's boundaries \Comment{$\mathbf{x}\in\mathbb{R}^n$ but domain is $\textbf{ D }\subset\mathbb{R}^n$}
\For{$i=1,\dots,n$}
	\State {l}$\gets${$i^{th}$ lower bound}
	\State {u}$\gets${$i^{th}$ upper bound}
	\State $x_N\gets\frac{\mathbf{x}^{(i)}-\textit{l}}{u-l}$\Comment{normalise $i^{th}$ component of $\mathbf{x}$ in $[0,1]$}
	\State $x_{R}\gets${rounds} $\mathbf{x}^{(i)}$ {to the nearest integer towards $0$}
	\If{$x_N > 1$}%\Comment{Toroidal transformation}
		\State $x_N\gets x_N-x_R$
	\ElsIf{$x_N < 0$}
		\State $x_N\gets 1 - \left|x_N-x_R\right|$
	\EndIf	
	\State $\mathbf{x_{corrected}}^{(i)}\gets{l}+X_N\cdot\left(u-l\right)$\Comment{scale the corrected value back to \textbf{D}}
\EndFor
\State \textbf{Output} $\mathbf{x_{corrected}}$
%\EndFunction
\end{algorithmic}
\end{center}
\end{algorithm}
